Anatomically Detailed Simulation of Human Torso

Existing digital human models approximate the human skeletal system using rigid bodies connected by rotational joints. While the simplification is considered acceptable for legs and arms, it significantly lacks fidelity to model rich torso movements in common activities such as dancing, Yoga, and various sports. Research from biomechanics provides more detailed modeling for parts of the torso, but their models often operate in isolation and are not fast and robust enough to support computationally heavy applications and large-scale data generation for full-body digital humans. This paper proposes a new torso model that aims to achieve high fidelity both in perception and in functionality, while being computationally feasible for simulation and optimal control tasks. We build a detailed human torso model consisting of various anatomical components, including facets, ligaments, and intervertebral discs, by coupling efficient finite-element and rigid-body simulations. Given an existing motion capture sequence without dense markers placed on the torso, our new model is able to recover the underlying torso bone movements. Our method is remarkably robust that it can be used to automatically "retrofit" the entire Mixamo motion database of highly diverse human motions without user intervention. We also show that our model is computationally efficient for solving trajectory optimization of highly dynamic full-body movements, without relying on any reference motion. Physiological validity of the model is validated against established literature.

==> notes.tex <==
Realistic modeling and simulation of human body movements have a wide range of applications from entertainments to robotics to medicine. Conventionally, human models used in computer graphics focus on visual realism while those used in biomechanics focus on anatomical realism. With recent advances in modeling, simulation and generative models, new simulated human models that achieve both high fidelity in perception and in function, while still robust and computationally efficient are closer to the horizon.

Human skeletal system is typically approximated as an articulated rigid body system, with hinge or ball-and-socket joints connecting the body segments. While the simplification can be acceptable for legs and arms, the human torso is significantly more complex. For example, the vertebrae bones can rotate to provide spine flexibility and can also translate to absorb compressive impact along the spinal column. Similarly, the shoulder complex manifests complicated range of motion (RoM) governed by multiple non-linear inter-bone constraints. Using only rotational joints to model the human torso limits our ability to visualize and synthesize realistic and detailed upper-body-rich human activities, such as gymnastics, yoga, and baseball pitching. 

This paper takes a step toward building a biomechanically realistic torso model that goes beyond the chain-of-rigid-bodies structure. Instead of connected by joints, the vertebral bones of our spine model are connected and regulated by discs, ligaments and facets, where we simulate the elastic discs with finite-element method based on the Projective Dynamics \cite{}, two-way coupled with the bones, and simulate the ligaments and facets as non-linear inequality constraints in an LCP (Linear Complementary Problem) framework. Similarly, the movement of scapula, clavicle, and rib cage are also subject to their own non-linear constraints. The interactions between all elements collectively determine the RoM of our skeletal model, as well as its passive dynamical properties such as elastic damping and constraint strength. The model parameters are automatically adjusted such that the simulated torso can match the real human's RoM.

Our torso model is kinematically and dynamically accurate and is two-way coupled with the rest of the human body through boundary conditions, easily swappable with the simplified torso of existing human models. We show that existing motion capture (mocap) data can be "retrofit" to obtain realistic and detailed torso and shoulder movements that match the movements of limbs in the mocap data. Because this problem is inherently under determined, the dynamic constraints imposed by our model are necessary for solving physically and anatomically plausible torso motions. As such, our method can serve as a principled tool to enrich motion capture data by adding unobserved skeletal movements. We also show that our model is computationally fast enough for optimal control with physics simulation. We optimize a sequence of control force from the torso to produce plausible motions, without using any reference data. In comparison to simplified torso, our model can generate much more momentum, on par with real human's capability. 

Perhaps the most interesting applications enabled by our model lie in medicine and healthcare. Back pain is a common illness among old people. MRI is limited to diagnose the spine state in action. A model that can predict the detailed disc deformation, ligaments tension, vertebrae positions, conditioned on the observable movement of the person is very valuable. \karen{Will polish it if we can deliver.}

We evaluate our model by reaffirming findings from biomechanics literature, demonstrating the biological validity of our model and its potentials to be used for biomedical analysis. \karen{Say a few concrete examples.}


% The discs are tightly attached to the bones with negligible inertial effects comparing to the bones \karen{fact check}. \yifeng{I think the reason is not quasi-static and negligible inertial. this is just variational integration where we need to minimize $E(x)$ at each sim step.} As such, we can assume that discs are quasi-static and at equilibrium at any time instance:
% \begin{equation}
% \label{eq:quasi_fem}  \mathbf{f}(\mathbf{x}) \equiv - \nabla_{\mathbf{x}} E(\mathbf{x}) = \mathbf{0}
% \end{equation}
% where $E(\mathbf{x})$ is the elastic energy, accounting for the material properties of the disc which depend on the constitutive model, elasticity, and the volume preservation. The elastic energy is non-linear in general. To solve Equation~(\ref{eq:quasi_fem}), we linearize it via Taylor expansion $\mathbf{f}(\mathbf{x}) \simeq\mathbf{f}(\mathbf{x}_0) +\nabla\mathbf{f}(\mathbf{x} - \mathbf{x}_0) $ where the gradient is evaluated at $\mathbf{x}=\mathbf{x}_0$. We iterate between updating the linearization and solving the linear system until the system converges:
% \begin{equation}
% \label{eq:quasi_fem2} \mathbf{K}\mathbf{x}_{i+1} = \mathbf{K}\mathbf{x}_i - \mathbf{f}(\mathbf{x}_i)
% \end{equation}
% where $\mathbf{K} = \nabla\mathbf{f}(\mathbf{x}) = -\nabla^2E(\mathbf{x})$ is the stiffness matrix evaluated at $\mathbf{x} = \mathbf{x}_i$. \yifeng{are these sentences just Newton's method?} The elastic energy is defined by the sum of many energy terms: $E(\mathbf{x}) = \sum_j E_j(\mathbf{x})$, where each term is associated with an individual constraint. \yifeng{what are these constraints, some subspace? and we need to project into these subspsaces?} The evaluation of the stiffness matrix and its inverse is prohibitively costly. Therefore, we adop the idea of Projective Dynamics~\cite{XXX} to reduce the computational cost. According to the Projective Dynamics, the evaluation of each elastic energy term can be decoupled into investigating a non-linear constraint manifold and measuring a quadratic distance \karen{What do you mean by "investigating"?}:
% \begin{equation}
% \label{eq:projection_energy}E_j(\mathbf{x}) = \min_{\mathbf{m}_j \in \mathcal{M}_j}\frac{1}{2}k_j||\mathbf{A}_j\mathbf{x} - \mathbf{m}_j||^2
% \end{equation}
% where $\mathcal{M}_j$ is the constraint manifold, $\mathbf{m}_j$ is a projection of $\mathbf{A}_j\mathbf{x}$ onto the constraint manifold \karen{$\mathbf{A}$ is not defined.}. $\mathbf{A}_j$ and $\mathcal{M}_j$ depend on the constitutive model and they are constant during simulation. Once we find the projection $\mathbf{m}_j$ for each constraint by solving the minization problem on the Equation~(\ref{eq:projection_energy}), the quadratic distance serves as the elastic energy of which the stiffness matrix (the Hessian) remains constant and we can accelerate solving the system of linear equations by pre-factorization such as Cholesky decomposition. Incorporating the Equation~(\ref{eq:projection_energy}) into the Equation~(\ref{eq:quasi_fem2}) yields: \yifeng{did you come up with using this factorization or did the original paper use this already? If the latter, no need to discuss $L$ in detail and just say we can solve fast.}
% \begin{equation}
% \label{eq:fem_simple}\mathbf{L}\mathbf{x}_{i+1} = \mathbf{d}(\mathbf{x}_i)
% \end{equation}
% where $\mathbf{L} = \sum_jk_j\mathbf{A}_j^{\rm T} \mathbf{A}_j$ and $\mathbf{d}(\mathbf{x}_i) = \sum_j\mathbf{A}_j^{\rm T}\mathbf{m}_j(\mathbf{x}_i)$ \karen{In general, the Projective Dynamics described above is hard to understand if the readers didn't know it before. We can add mode details and move it to Appendix, if we didn't add anything novel to the original algorithm}.
% \yifeng{I think in general it's good to give a quick overview of projective dynamics, but more importantly followed by how our problem maps to the key concepts in projective dynamics. For example, what are the non-linear constraints in our problem that have biomechanics meanings, and how do we design the distance metric function} 

% We incorporate three energy functions to model the behaviors of discs: $E_{\rm background}(\mathbf{x})$, $E_{\rm vol}(\mathbf{x})$, and $E_{\rm pos}(\mathbf{x}, \mathbf{T})$. $E_{\rm background}(\mathbf{x})$ is a strain energy which explains the background isotropic elasticity of the disc \karen{What does "background" here mean}, $E_{\rm vol}(\mathbf{x})$ is a volume preservation term, and $E_{\rm pos}(\mathbf{x},\mathbf{T})$ describes the positional constraints that attach the disc to the bone. The transformation matrices of the vertebrae bones $\mathbf{T} =(\mathbf{T}_1,\mathbf{T}_2, \cdots, \mathbf{T}_{23})\in \mathbb{R}^{4\times4\times23}$ serve as boundary conditions for Equation~(\ref{eq:quasi_fem}). The reaction to the positional constraint forces $-\mathbf{f}_{\rm pos}(\mathbf{x}, \mathbf{T})$ is applied to the adjacent bone (See Figure~\ref{fig:vertebrae_bone}).
% We detail the derivation of each constraint in Appendix \karen{Each? Each of the 23 position constraints? Aren't they the same?}. \yifeng{need the definition of $f_{pos}$, or equivalently $E_{pos}$. How does our $E_{pos}$ correspond to projective dynamics form with the $\delta$ functions? \url{https://www.projectivedynamics.org/Projective_Dynamics/index.html } Equation 15 to 17.}


%Models of human torso for animation purposes usually optimize for visual realism and computational efficiency without stressing anatomical correctness, while torso models for biomechanics are often anatomically more detailed but could nevertheless compromise robustness and speed. We build a detailed human torso model consisting of various anatomical components such as facets, ligaments, and intervertebral discs, by coupling efficient finite-element and rigid-body simulations. Given underdetermined optical motion capture as input, our new model is robust enough to be able to recover the underlying torso bone movements for a large variety of motions. We are also able to solve trajectory optimization for highly dynamic movements, without using any captured motion, with the torso physically simulated by our model. Physiological validity of the model is validated against established literature.

==> tex/4-retrofication.tex <==
\section{Motion Retrofication}

Motion retrofication is a problem of enriching the detailed upper body motions from  standard motion capture system such as AMASS and CMU motion capture system. There exist few motion capture markers on the upper body and they are not enough to capture the features of the torso movements. This is critical when we are dealing with upper-body-rich human motions such as gymnastics, yoga, ballet and jumping.

Given the sequence of motion capture markers and their labels, our goal is to retrofit the upper body motions such that the model fits the 3D marker positions as close as possible. Unlike motion reconstruction where plenty of markers are given, our problem is overly under-determined system where we observe small numbers of marker positions compared to the degrees of freedom (dofs) of the upper body. In this context we adopt our upper body dynamics, capable of filling up the remain dofs under the hypothesis where the upper body should be physically and anatomically plausible.

In this section we present a novel two-stage framework that enables the motion retrofication of the torso that combines steady-state analysis with a following trajectory optimization that learns to actuate the upper body. The 


which can be parallelized 


This fact is distinct the motion retrofication from motion reconstruction whereAs our problem is overly 
our problem is overly under-determined system where t
stadard motion capture marker set such as AMASS marker set and CMU marker set, we the positions of shoul

The torso movements are passive. In this context we want to utilize our upper body simulation as a passive 



enriching motion capture data. 

Reconstructs detailed upper body motion from standard mocap system in which torso movements are unobservable.
Retrofits mocap dataset, AMASS, to improve its upper body motion.
Physically simulates upper-body-rich human motions such as baseball, gymnastics, yoga, ballet, high jump, unachievable by previous simple human models.
